Harnessing LLMs Without Surrendering Control: Delegation Boundaries in Visual Data Storytelling Authoring

Despite the emergence of large language models (LLMs) for visual data storytelling workflows, there are open questions about how authors decide what activities or tasks to entrust to them and what should be "protected" or maintained under human control. To investigate this, we interviewed a cohort of 12 expert visual data storytellers. Our analysis shows that participants rarely treated LLMs as autonomous storytellers. Instead, they tend to selectively delegate execution-oriented tasks to LLMs while retaining control over activities that shape narrative intent and story meaning. Our findings show that LLM assistance is most productive after human seeding and constraint-setting, and that it shifts labor from production to verification. We discuss design implications for boundary-aware authoring tools, data-grounded generation, low-fidelity ideation, and reporting practices for LLM-based visualization research. Supplemental materials for this paper are available at https://osf.io/hcnp6.

==> 99.tex <==
% appendix
\section{Appendices}
% \section{Participant Demographics}
% \label{appendix:participant_demographics}
% \begin{table}[h]
%     \centering
%     \small
%     \caption{Participant demographics.}
%     \setlength{\tabcolsep}{3pt}
%     \begin{tabular}{l l p{2.6cm} c l c}
%     \toprule
%     ID & Area & Role & Experience (yrs) & LLM Usage & PVIS$^{\ast}$\\
%     \midrule
%     P1  & USA        & Both (research \& practice) & 6 & Daily & 1 \\
%     P2  & USA        & Academic researcher & 5 & Daily & 1 \\
%     P3  & USA        & Industry practitioner & 4 & Occasionally  & 1 \\
%     P4  & USA        & Both (research \& practice)            & 3 & Weekly& 1 \\
%     P5  & USA        & Industry practitioner & 3 & Daily & 1 \\
%     P6  & China$^{\dagger}$ & Both (research \& practice)        & 2 & Daily & 1 \\
%     P7  & China$^{\dagger}$ & Adjacent field & 1 & Daily & 1 \\
%     P8  & Korea         & Academic researcher & 5 & Daily & 0 \\
%     P9  & Singapore         & Academic researcher & 5 & Daily & 0 \\
%     P10 & China         & Industry practitioner  & 7 & Daily & 1 \\
%     P11 & China         & Academic researcher & 3 & Weekly& 0 \\
%     P12 & China         & Industry practitioner & 2 & Daily & 1 \\
%     \bottomrule
%     \end{tabular}
%     \vspace{2pt}
%     \begin{minipage}{\linewidth}
%     {\footnotesize $^{\ast}$Indicates prior participation in or awards from the IEEE PacificVis visual data storytelling contest. $^{\dagger}$Participants from Hong Kong.}
%     \end{minipage}
    
%     \label{tab:participants}
% \end{table}

% \section{Coding Framework}
% \label{appendix:coding-framework}
% \begin{table*}[t]
%     \centering
%     \caption{\textbf{Coding framework for analyzing LLM-mediated narrative visualization authoring.}
%     We coded each meaning unit along six analytic dimensions. The dimensions were used relationally:
%     use cases were compared with delegation levels, risks were compared with verification strategies,
%     and authorial-control codes were interpreted together with boundary rationales.}
%     \label{tab:coding-framework}
%     \small
%     \setlength{\tabcolsep}{4pt}
%     \renewcommand{\arraystretch}{1.18}
    
%     \begin{tabularx}{\textwidth}{
%         >{\raggedright\arraybackslash}p{0.17\textwidth}
%         >{\raggedright\arraybackslash}p{0.33\textwidth}
%         >{\raggedright\arraybackslash}X
%     }
%     \toprule
%     \textbf{Dimension} &
%     \textbf{Analytic purpose} &
%     \textbf{Representative codes} \\
%     \midrule
    
%     \tagUC\ \textbf{LLM use cases} &
%     Identifies where LLMs entered participants' narrative visualization and data storytelling workflows. These codes capture the task context before interpreting whether the task was delegated, constrained, or protected. &
%     \tagUCx{Ideation}
%     \tagUCx{StoryStruct}
%     \tagUCx{LanguageRefine}
%     \tagUCx{AudienceAdapt}
%     \tagUCx{DataSearch}
%     \tagUCx{AssetGen}
%     \tagUCx{TechImpl}
%     \tagUCx{CritiqueReview} \\
    
%     \addlinespace[0.35em]
    
%     \tagDL\ \textbf{Delegation levels} &
%     Captures how much authority participants gave to LLMs in a specific task. This dimension supports the delegation boundary map by distinguishing protected decisions from consultative, refinement, drafting, and execution-oriented uses. &
%     \tagDLx{NoUse}
%     \tagDLx{Consult}
%     \tagDLx{Critique}
%     \tagDLx{Refine}
%     \tagDLx{DraftGen}
%     \tagDLx{FullExec} \\
    
%     \addlinespace[0.35em]
    
%     \tagPR\ \textbf{Perceived risks} &
%     Captures concerns that emerged when LLMs were used or considered, including not only factual errors but also process-level and authorship-level risks. &
%     \tagPRx{DataTrust}
%     \tagPRx{Hallucination}
%     \tagPRx{ClaimOverreach}
%     \tagPRx{ContextLoss}
%     \tagPRx{CogAnchor}
%     \tagPRx{Homogenization}
%     \tagPRx{SkillDecay}
%     \tagPRx{Privacy} \\
    
%     \addlinespace[0.35em]
    
%     \tagVS\ \textbf{Verification strategies} &
%     Identifies how participants checked, constrained, revised, or rejected LLM outputs. These codes show how LLM use shifted effort from production to verification and curation. &
%     \tagVSx{CrossSource}
%     \tagVSx{DataGrounding}
%     \tagVSx{PromptConstraint}
%     \tagVSx{OutputObs}
%     \tagVSx{CodeRunTest}
%     \tagVSx{HumanJudgment}
%     \tagVSx{ManualRewrite}
%     \tagVSx{IterativeRef} \\
    
    
%     \addlinespace[0.35em]
    
%     \tagBR\ \textbf{Boundary rationales} &
%     Explains why participants delegated or protected specific tasks. These codes connect task characteristics to underlying judgments about risk, expertise, originality, evidence, and responsibility. &
%     \tagBRx{Mechanical}
%     \tagBRx{TimeSaving}
%     \tagBRx{ExpertiseGap}
%     \tagBRx{LowStakes}
%     \tagBRx{IntentSensitivity}
%     \tagBRx{ClaimSensitivity}
%     \tagBRx{Originality}
%     \tagBRx{Accountability} \\
    
%     \addlinespace[0.35em]
    
%     \tagAC\ \textbf{Authorial control} &
%     Captures how participants maintained authorship and responsibility when using LLMs. These codes identify the decisions participants considered central to the story, the evidence, the visual argument, or the audience relationship. &
%     \tagACx{IntentSeeding}
%     \tagACx{FlowMastery}
%     \tagACx{ClaimOwnership}
%     \tagACx{VisualOwnership}
%     \tagACx{VoiceOwnership}
%     \tagACx{Curation}
%     \tagACx{AudienceResponsibility}
%     \tagACx{FinalAccountability} \\
    
%     \bottomrule
%     \end{tabularx}
    
%     \vspace{0.35em}
%     \begin{minipage}{0.98\textwidth}
%     \footnotesize
%     \textit{Note.} Codes were non-exclusive. A single transcript segment could receive multiple codes
%     when a participant discussed, for example, an LLM use case, a delegation decision, a risk, and a
%     verification strategy in the same response. The full codebook, coded excerpts, and participant-level
%     matrices are provided in the supplementary material.
%     \end{minipage}
%     \vspace{-0.6em}
% \end{table*}

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January and March 2023

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unix-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

